The impact of superconductivity and the Hall effect in models of magnetized neutron stars

Equilibrium configurations of the internal magnetic field of a pulsar play a key role in modeling astrophysical phenomena, from glitches to gravitational wave emission. In this paper we present a numerical scheme for solving the Grad-Shafranov equation and calculating equilibrium configurations of pulsars, accounting for superconductivity in the core of the neutron star, and for the Hall effect in the crust of the star. Our numerical code uses a finite-difference method in which the source term appearing in the Grad-Shafranov equation, used to model the magnetic equilibrium is nonlinear. We obtain solutions by linearizing the source and applying an under-relaxation scheme at each step of computation to improve the solver's convergence. We have developed our code in both C++ and Python, and our numerical algorithm can further be adapted to solve any nonlinear PDEs appearing in other areas of computational astrophysics. We produce mixed toroidal-poloidal field configurations, and extend the portion of parameter space that can be investigated with respect to previous studies. We find that even in the more extreme cases the magnetic energy in the toroidal component does not exceed approximately 5\% of the total. We also find that if the core of the star is superconducting, the toroidal component is entirely confined to the crust of the star, which has important implications for pulsar glitch models which rely on the presence of a strong toroidal field region in the core of the star, where superfluid vortices pin to superconducting fluxtubes.

==> abstract.tex <==
Neutron star matter is often represented by a barotropic equation of state. Whether magnetic field in barotropic stars are at all stable has caught much attention recently. Thus, finding equilibrium configurations of the magnetic field in neutron stars is an important astrophysical problem for understanding its long-term evolution. This requires us to solve the Laplacian like Grad-Shafranov equation for a two-dimensional plasma, which is a second-order nonlinear partial differential equation. In this paper, we present an iterative numerical scheme for solving the Grad-Shafranov equation in spherical coordinates and where possible, show comparisons with known results. \textcolor{red}{Our code is python based which uses \texttt{numpy} vectorization, improving its performance speed by many folds}. The numerical method uses a finite-difference scheme. An under-relaxation applied at each step of computation have shown to improve the convergence of the solution significantly. This method can also be adapted to solve any nonlinear PDE appearing in other areas of computational physics.
